Data fusion for a multi-scale model of a wheat leaf surface: a unifying approach using a radial basis function partition of unity method

Realistic digital models of plant leaves are crucial to fluid dynamics simulations of droplets for optimising agrochemical spray technologies. The presence and nature of small features (on the order of 100$\mathrm{\mu m}$) such as ridges and hairs on the surface have been shown to significantly affect the droplet evaporation, and thus the leaf's potential uptake of active ingredients. We show that these microstructures can be captured by implicit radial basis function partition of unity (RBFPU) surface reconstructions from micro-CT scan datasets. However, scanning a whole leaf ($20\mathrm{cm^2}$) at micron resolutions is infeasible due to both extremely large data storage requirements and scanner time constraints. Instead, we micro-CT scan only a small segment of a wheat leaf ($4\mathrm{mm^2}$). We fit a RBFPU implicit surface to this segment, and an explicit RBFPU surface to a lower resolution laser scan of the whole leaf. Parameterising the leaf using a locally orthogonal coordinate system, we then replicate the now resolved microstructure many times across a larger, coarser, representation of the leaf surface that captures important macroscale features, such as its size, shape, and orientation. The edge of one segment of the microstructure model is blended into its neighbour naturally by the partition of unity method. The result is one implicit surface reconstruction that captures the wheat leaf's features at both the micro- and macro-scales.

==> src/nomenclature.tex <==
\begin{table}[h]
    \centering
    \caption{Nomenclature}
    \label{tab:nomenclature}
    \begin{tabular}{lp{0.6\linewidth}}
        \toprule
        Term & Usage and/or meaning \\
        \midrule
        world coordinates & the coordinate system of the macro-scale point cloud of the whole leaf \\
        leaf coordinates & the constructed coordinate system following the medial axis of the leaf \\
        RBFPUM & Radial Basis Function Partition of Unity Method \\
        $\mathcal{T}$ & the coordinate transform from world to leaf coordinates \\
        $\mathcal{F}$ & the implicit RBFPUM interpolant of the micro-scale CT data \\
        $\mathcal{F}_i$ & a local interpolant on a partition of unity subdomain \\
        $\mathcal{G}$ & a multi-scale RBFPUM interpolant \\
        $\mathcal{H}$ & the explicit interpolant of the point cloud in leaf coordinates \\
        $\vec{x}$, $\vec{y}$, $\vec{z}$ & points in world, leaf, and micro-CT coordinates, respectively \\
        $\vec{c}_i, r_i$ & the centre and radius of a PUM subdomain \\
        $w(\tau)$ & PUM weight function \\
        $w_i(\vec{x})$ & PUM weight function, shifted and scaled to the $i$-th subdomain \\
        $\vec{s}_i^q$ & the displacement vector of the $q$-th copy of subdomain $i$ \\
        \bottomrule
    \end{tabular}
\end{table}

